Feature Compression for Rate Constrained Object Detection on the Edge

Recent advances in computer vision has led to a growth of interest in deploying visual analytics model on mobile devices. However, most mobile devices have limited computing power, which prohibits them from running large scale visual analytics neural networks. An emerging approach to solve this problem is to offload the computation of these neural networks to computing resources at an edge server. Efficient computation offloading requires optimizing the trade-off between multiple objectives including compressed data rate, analytics performance, and computation speed. In this work, we consider a "split computation" system to offload a part of the computation of the YOLO object detection model. We propose a learnable feature compression approach to compress the intermediate YOLO features with light-weight computation. We train the feature compression and decompression module together with the YOLO model to optimize the object detection accuracy under a rate constraint. Compared to baseline methods that apply either standard image compression or learned image compression at the mobile and perform image decompression and YOLO at the edge, the proposed system achieves higher detection accuracy at the low to medium rate range. Furthermore, the proposed system requires substantially lower computation time on the mobile device with CPU only.

==> unused_contents.tex <==
%%%%%%%%%%%%%%%% Runtime Table (more details) %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp]
\begin{tabular}{l|lc|lc|lcc}
\hline
                                                                              &                   & \cite{balle2018variational} + YOLO &         & BPG + YOLO &                   & C4\_D3 & C4\_D4 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Mobile Device\\ (CPU)\end{tabular}} & Main Encoder      & 376.2         & Encoder & 183.87     & YOLO Pre-split    & 46.25  & 67.37  \\
                                                                              & Hyper Encoder     & 5.026         &         &            & Hyper Encoder     & 0.899  & 0.640  \\
                                                                              & Arithmetic Encoding & 34.23         &         &            & Arithmetic Encoding & 15.94  & 8.244  \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Edge Server\\ (GPU)\end{tabular}}   & Hyper Decoder     & 0.349         & Decoder & 84.39      & Hyper Decoder     &  0.265 & 0.253  \\
                                                                              & Main Decoder      & 1.475         &         &            &                   &        &        \\
                                                                              & YOLO              & 7.387         & YOLO    & 7.387      & YOLO Post-split   & 6.742  & 5.298  \\ \hline \hline
Total time (ms)                                                                &                   & 424.7         &         & 275.6    &                   &  70.1  & 81.8 \\ \hline
\end{tabular}
\caption{Breakdown of runtime (milliseconds) per image for proposed model and baselines. C4\_D3 and C4\_D4 refer to models with channel reduction to $N_{r}=4$ and split point at D3 and D4, respectively.}
\label{table:runtime}
\end{table*}


%%%%%%%%%%%%%%%%  FLOP Table %%%%%%%%%%%%%%%%

\begin{table*}[htbp]
\centering

\begin{tabular}{l|lc|lcc}
\hline
                                                                              &                   & \cite{balle2018variational} + YOLO &                     &
                                                                              C4\_D3 & C4\_D4 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Mobile Device\\ (CPU)\end{tabular}} & Main Encoder      &30.18     &YOLO Pre-split    & 3.59  & 6.54  \\
                                                                              & Hyper Encoder     &3.35      & Hyper Encoder     & $4\times10^{-3}$  & $9\times10^{-4}$  \\
                                                                              & Arithmetic Encoding & -      & Arithmetic Encoding & -  & -  \\ \hline
                                                                               
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Edge Server\\ (GPU) \\ \\ \end{tabular}}   & Hyper Decoder     &          16.20& Hyper Decoder     & $1.5\times10^{-2}$  & $1.5\times10^{-2}$  \\
                                                                              & Main Decoder      &          120.62&          YOLO Post-split   & 12.01  & 9.06
                                                                            &    &YOLO              &          15.6    &                  &        &   \\  \hline \hline
GFLOP                                                                &                   & 185.95        &                        & 15.62   & 15.62 \\ \hline
\end{tabular}
\hspace{0.5}\caption{Giga floating point operations (GFLOP) per image for proposed model and baselines measured using \cite{thop}. The FLOP count of BPG and arithmetic encoding cannot be obtained using \cite{thop} and are not reported.}
\label{table:flop}
\end{table*}
